OneDayAgent: Towards a Long-Horizon Harness for Autonomous Agents

LLM agents are increasingly applied to open-ended everyday requests that span work, study, and life. These tasks are long-horizon, cross-environment, and multimodal, forcing the agent to preserve goals and constraints across many steps while navigating heterogeneous tools and attachments. While prior work has addressed individual failure modes such as goals drift, states loss, and context overflow, whether a single harness can manage them jointly and remain effective across backends has received less study. We present OneDayAgent, a long-horizon harness for autonomous agents. OneDayAgent turns an open-ended request into a managed execution process that decomposes tasks into bounded subtasks, maintains execution memory under context pressure, and verifies and repairs the final deliverable. We evaluate OneDayAgent on AgentIF-OneDay across 104 tasks. With the GLM-5.2 backend, OneDayAgent sets a new state of the art with an overall score of 0.821. The same harness runs across five backend LLMs from three model families, indicating the harness generalizes across backends without tuning, even as different models induce distinct execution styles under the same workflow.

==> tables/experiment_setup.tex <==
\begin{table*}[t]
\centering
\small
\renewcommand{\arraystretch}{1.35}
\setlength{\tabcolsep}{5pt}
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{Y}{>{\raggedright\arraybackslash}X}
\begin{tabularx}{\textwidth}{L{0.12\textwidth} L{0.18\textwidth} Y}
\toprule
\textbf{Group} & \textbf{Setting} & \textbf{Value} \\
\midrule
\multirow{2}{=}{Benchmark}
& Suite and score & AgentIF-OneDay, 104 tasks, 767 instance-level rubric points; per-task normalized score in $[0,1]$ averaged over all tasks \\
& Baselines & Official AgentIF-OneDay general-purpose agent baselines (Minimax-Agent, ChatGPT-Agent, Genspark, Manus, AutoClaw) and an additional Codex run with GPT-5.5 medium \\
\addlinespace[2pt]
\midrule
\multirow{3}{=}{Backend LLMs}
& Main backend & GLM-5.2 \\
& Backend variants & GLM-5.2, Gemini-3.1-Pro-Preview, Qwen3.5-397B-A17B, Qwen3.6-27B, Qwen3.5-9B \\
& Decoding & Official recommended settings for daily and coding tasks: temperature 1.0, top-$p$ 0.95, max tokens 128K, presence penalty 0.0; all backends use thinking mode by default. \\
\addlinespace[2pt]
\midrule
\multirow{2}{=}{Judge}
& Framework & Official AgentIF-OneDay LLM-as-judge pipeline \\
& Judge model & Gemini-3.1-Pro-Preview; temperature 0.1; max tokens 65,536 \\
\addlinespace[2pt]
\midrule
\multirow{3}{=}{Harness}
& Execution budget & 200 ReAct iterations; 7200-second task timeout; 128K active context budget \\
& Long-horizon controls & At most 6 subtasks; failed subtasks use 3 total attempts; global verification and repair enabled \\
& Context management & Compression at 0.9$\times$ context budget; recent 3 rounds kept verbatim \\
\bottomrule
\end{tabularx}
\caption{\textbf{Experiment setup.}
We summarize the benchmark, backend LLMs, judge configuration, and core harness settings used in the reported experiments.
Detailed tool interfaces and full harness configuration are provided in Appendix Tables~\ref{tab:tool_environment_full} and~\ref{tab:harness_configuration}.}
\label{tab:experiment_setup}
\end{table*}


==> tables/main1.tex <==
% ==================== Level-4 长序列表格（暂未填充数据，保留备用） ====================
% \begin{table}[t]
% \centering
% \caption{Success rates (\%) on LabUtopia Level-4 long-horizon tasks.
% SP = single-stage primitive success rate; A1--A7 = sub-steps in the task sequence.}
% \label{tab:level4_results}
% \renewcommand{\arraystretch}{1.18}
% \resizebox{0.95\linewidth}{!}{%
% \begin{tabular}{l l c cccccccc}
% \toprule
% \multirow{2}{*}{\textbf{Task}} & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Size}}
% & \multicolumn{8}{c}{\textbf{Success Rate (\%)}} \\
% \cmidrule(lr){4-11}
% & & & SP & A1 & A2 & A3 & A4 & A5 & A6 & A7 \\
% \midrule
% \multicolumn{11}{l}{\textit{Clean Beaker}} \\[2pt]
%  & ACT \cite{fu2024mobile}                         & $<$1B & 14.0 & 99.3 & 51.9 & 43.3 & 42.5 & 12.3 & 10.6 & 1.6 \\
%  & DP \cite{chi2025diffusion}                      & $<$1B & 2.5  & 92.7 & 8.1  & 1.3  & 0.0  & 0.0  & 0.0  & 0.0 \\
%  & SmolVLA \cite{shukor2025smolvla}                & $<$1B & --   & --   & --   & --   & --   & --   & --   & --  \\
%  & $\pi_0$ \cite{black2024pi_0}                    & 3B    & --   & --   & --   & --   & --   & --   & --   & --  \\
%  & $\pi_{0.5}$ \cite{intelligence2025pi_}          & 3B    & --   & --   & --   & --   & --   & --   & --   & --  \\
%  & \rowcolor{blue!6} \textbf{OneDayAgent (Ours)}        & 3B    & --   & --   & --   & --   & --   & --   & --   & --  \\
% \midrule
% \multicolumn{11}{l}{\textit{Drying Beakers}} \\[2pt]
%  & ACT \cite{fu2024mobile}                         & $<$1B & 6.3  & 81.3 & 42.0 & 19.7 & 9.3  & 3.5  & 1.2  & 0.0 \\
%  & DP \cite{chi2025diffusion}                      & $<$1B & 2.0  & 76.0 & 32.0 & 26.3 & 0.0  & 0.0  & 0.0  & 0.0 \\
%  & \rowcolor{blue!6} \textbf{OneDayAgent (Ours)}        & 3B    & --   & --   & --   & --   & --   & --   & --   & --  \\
% \midrule
% \multicolumn{11}{l}{\textit{Liquid Fusion}} \\[2pt]
%  & ACT \cite{fu2024mobile}                         & $<$1B & 8.3  & 96.3 & 57.6 & 46.7 & 42.5 & 12.3 & 10.6 & 1.6 \\
%  & DP \cite{chi2025diffusion}                      & $<$1B & 6.7  & 93.5 & 12.3 & 8.3  & 0.0  & 0.0  & 0.0  & 0.0 \\
%  & \rowcolor{blue!6} \textbf{OneDayAgent (Ours)}        & 3B    & --   & --   & --   & --   & --   & --   & --   & --  \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}


\begin{table}[t]
\centering
\caption{Success rates (\%) on AutoBio benchmark tasks across three difficulty levels.}
\label{tab:autobio_results}
\vspace{-2mm}
\small
\renewcommand{\arraystretch}{1.18}
% tabcolsep 控制列间距，可调整（默认6pt，增大则表格更宽）
\setlength{\tabcolsep}{8pt}
\begin{tabular}{l cccccc}
\toprule
\multirow{2}{*}{\textbf{Task}} & \multicolumn{6}{c}{\textbf{Success Rate (\%)}} \\
\cmidrule(lr){2-7}
 & SmolVLA & X-VLA & $\pi_0$ & $\pi_{0.5}$ & UniVLA & \textbf{OneDayAgent (Ours)} \\
\midrule
\multicolumn{7}{l}{\textit{Easy}} \\[2pt]
Close thermal cycler lid     & 100 & 99 & 100 & 100 & -- & -- \\
Open thermal cycler lid      &  97 & 100 &  98 &  95 & -- & -- \\
Pick up centrifuge tube      &  42 & 91 &  56 &  82 & -- & -- \\
\midrule
\multicolumn{7}{l}{\textit{Medium}} \\[2pt]
Unscrew centrifuge tube cap  &  19 & 0  &  17 &   8 & -- & -- \\
Aspirate with pipette        &  71 & 0  &  32 &  20 & -- & -- \\
Transfer centrifuge tube     &  26 & 7  &  44 &  36 & -- & -- \\
\midrule
\multicolumn{7}{l}{\textit{Hard}} \\[2pt]
Screw on centrifuge tube cap &   1 & 0  &   0 &   7 & -- & -- \\
Operate thermal mixer panel  &  0.2 & 0.3 &   5 &   0 & -- & -- \\
Load centrifuge rotor        &  16 & 3  &   9 &  13 & -- & -- \\
\bottomrule
\end{tabular}
\end{table}





















